Exploring Large Language Models in Resolving Environment-Related Crash Bugs: Localizing and Repairing

Software crash bugs cause unexpected program behaviors or even abrupt termination, thus demanding immediate resolution. However, resolving crash bugs can be challenging due to their complex root causes, which can originate from issues in the source code or external factors like third-party library dependencies. Large language models (LLMs) have shown promise in software engineering tasks. However, existing research predominantly focuses on the capability of LLMs to localize and repair code-related crash bugs, leaving their effectiveness in resolving environment-related crash bugs in real-world software unexplored. To fill this gap, we conducted the first comprehensive study to assess the capability of LLMs in resolving real-world environment-related crash bugs. We first systematically compare LLMs' performance in resolving code-related and environment-related crash bugs with varying levels of crash contextual information. Our findings reveal that localization is the primary challenge for resolving code-related crashes, while repair poses a greater challenge for environment-related crashes. Furthermore, we investigate the impact of different prompt strategies on improving the resolution of environment-related crash bugs, incorporating different prompt templates and multi-round interactions. Building on this, we further explore an advanced active inquiry prompting strategy leveraging the self-planning capabilities of LLMs. Based on these explorations, we propose IntDiagSolver, an interactive methodology designed to enable precise crash bug resolution through ongoing engagement with LLMs. Extensive evaluations of IntDiagSolver across multiple LLMs (including GPT-3.5, GPT-4, Claude, CodeLlama, DeepSeek-R1, and Qwen-3-Coder) demonstrate consistent improvements in resolution accuracy, with substantial enhancements ranging from 9.1% to 43.3% in localization and 9.1% to 53.3% in repair.

==> sections/discussion.tex <==
\section{Discussion}
\todo{respond to: The authors can also discuss the limitations and advantages of the ChatGPT-based solution with respect to the previous/traditional solutions, such as the following: R.Wu, et al., CrashLocator: Locating Crashing Faults based on Crash Stacks, Proc. International Symposium on Software Testing and Analysis (ISSTA'14), San Jose, CA, July 2014.}

\todo{respond to:The paper should discuss the difficulty level of localizing and fixing the different crashes' root causes. Not all crashes are equivalent, as some are simple to diagnose and fix, and others require specific conditions (like one particular complex object state) to happen. See, for instance, JCrashPack (Soltani, M., Derakhshanfar, P., Devroey, X. et al. A benchmark-based evaluation of search-based crash reproduction. Empir Software Eng 25, 96–138 (2020). https://doi.org/10.1007/s10664-019-09762-1) for a discussion on the matter.}


==> sections/setup_bak.tex <==
\section{Experimental Setup}


\subsection{Research Questions}
We focus on the following research questions in this work.

\begin{itemize}
    \item RQ1: How do \ourtool{} perform compared existing learning-based oracle generation techniques?
    
     \item RQ2: How do different mask strategies affect the performance of \ourtool{}?

    \item RQ3:  How does our ranking strategy contribute to the performance of \ourtool{}?
          
     \item RQ4: How does \ourtool{} perform on the top of different \llm{}s?

    \item RQ*: How does the number of fine-tuning epochs affect the effectiveness of \ourtool{}?  
    
\end{itemize}

\subsection{Datasets}
In line with existing work on assertion generation~\cite{DBLP:conf/icse/WatsonTMBP20,DBLP:conf/icse/YuLSR00L0W22, DBLP:conf/icse/DinellaRML22, DBLP:conf/icse/MastropaoloSCNP21, DBLP:journals/tse/Mastropaolo22}, we adopt the widely-used \atlas{} dataset in our experiment.  In particular, the original 


%mentioned there is no overlap between codet5 and the atlas testing 





\subsection{Compared Baselines}
We consider the following four state-of-the-art learning-based assertion generation techniques as baselines, including:

\begin{itemize}
\item \atlas~\cite{DBLP:conf/icse/WatsonTMBP20},  generates assertions by leveraging a basic sequence-to-sequence model; 

\item \irbased{}~\cite{DBLP:conf/icse/YuLSR00L0W22}, generates assertions with information retrieval techniques. In particular, we use the best variant of \irbased{}, which achieves the best accuracy by combining both information retrieval and deep learning techniques; 

\item \toga{}~\cite{DBLP:conf/icse/DinellaRML22}, first generates candidate assertions by template-based strategies and then trains a classifier to select the correct assertion;

\item \tfiveone{}~\cite{DBLP:conf/icse/MastropaoloSCNP21}, first pre-trains a T5 transformer model on a large corpus of code and text, and then fine-tune in downstream code related tasks.

\item \tfivetwo{}~\cite{DBLP:journals/tse/Mastropaolo22}, further improves \tfiveone{} by fine-tuning on more downstream tasks. 
\end{itemize}


\yiling{Maybe also include the seq2seq2 arxiv paper cited in toga as baseline as well (62\% accuracy).}


\subsection{Metric}
Following previous work~\cite{DBLP:conf/icse/WatsonTMBP20，DBLP:conf/icse/YuLSR00L0W22，DBLP:conf/icse/DinellaRML22，DBLP:conf/icse/MastropaoloSCNP21，DBLP:journals/tse/Mastropaolo22}, we use the exact matching accuracy as our major measurement. Particularly, a generated assertion would be considered as accurate only when it is exactly the same as the ground truth. For each technique, we calculate the ratio of  the accurate assertions to all its generated assertions in the testing set. 

\subsection{Experimental Procedure}


\textbf{How to run each RQ.}

\textbf{The implementation.}
%How do we set these pre-train models

\textbf{The Hyper parameters.}

\textbf{The Environment.}

